Algorithms for Internal Validation Clustering Measures in the Post Genomic Era

Inferring cluster structure in microarray datasets is a fundamental task for the -omic sciences. A fundamental question in Statistics, Data Analysis and Classification, is the prediction of the number of clusters in a dataset, usually established via internal validation measures. Despite the wealth of internal measures available in the literature, new ones have been recently proposed, some of them specifically for microarray data. In this dissertation, a study of internal validation measures is given, paying particular attention to the stability based ones. Indeed, this class of measures is particularly prominent and promising in order to have a reliable estimate the number of clusters in a dataset. For those measures, a new general algorithmic paradigm is proposed here that highlights the richness of measures in this class and accounts for the ones already available in the literature. Moreover, some of the most representative validation measures are also considered. Experiments on 12 benchmark datasets are performed in order to assess both the intrinsic ability of a measure to predict the correct number of clusters in a dataset and its merit relative to the other measures. The main result is a hierarchy of internal validation measures in terms of precision and speed, highlighting some of their merits and limitations not reported before in the literature. This hierarchy shows that the faster the measure, the less accurate it is. In order to reduce the time performance gap between the fastest and the most precise measures, the technique of designing fast approximation algorithms is systematically applied. The end result is a speed-up of many of the measures studied here that brings the gap between the fastest and the most precise within one order of magnitude in time, with no degradation in their prediction power. Prior to this work, the time gap was at least two orders of magnitude.

==> Introduction__old.tex <==
\chapter*{Introduction}
\label{chap:intro}
\addcontentsline{toc}{chapter}{Introduction} \pagenumbering{arabic}

The term bioinformatics, coined by Paulien Hogeweg, to indicated the application of statistics and computer science to the field of molecular biology, today assume various definition.
For instance, few examples from textbooks are: \vir{bioinformatics is the
rapidly developing area of computer science devoted to collecting, organizing, and
analyzing DNA and protein sequences}~\cite{SchenaShalonDavisBrown},  \vir{the use of computer methods
in studies of genomes}~\cite{CheScience96} and \vir{bioinformatics is the science of
refining biological information into biological knowledge using computers}~\cite{Wang98}.

In this wide and \vir{mystique} area of research the most pressing task now involves the analysis and interpretation of various types of data, including nucleotide and amino acid sequences, protein domains, and protein structures. The actual process of analyzing and interpreting data is referred to as \emph{computational biology}.


In this contest a useful and well established technology of study is the \emph{microarrays}.
Microarrays are part of a new and promising class of biotechnologies that allow the monitoring of expression levels in cells for thousands of gene simultaneously. Microarray experiments are increasingly being caried out in biological and medical research to address a wide range of problems, including the classification of tumors~\cite{Aliz00,AlonU1999,CLEST,golub99,Perou1999,Pollack99,Ross00}. A reliable and precise classification of tumors is essential for successful diagnosis and treatment of cancer. By allowing the monitoring of expression levels on a genomic scale, microarray experiments may lead to a more complete understanding of the molecular variations among tumors and hence to a finer and more reliable classification. An important statistical problem associated with tumor classification is the identification of new tumor classes using gene expression profiles. For these reasons clustering has become a popular data analysis
technique in genomic studies using gene-expression microarrays~\cite{CLEST,Kikuchi2003,McAdams-1995,Shmulevichbook}.
In Literature a large number of clustering algorithms has been proposed
and many of these have been applied to genomic data, the most famous are: K-means~\cite{JainDubes},
fuzzy c-means, self-organizing maps~\cite{Perrin2003,Sachs02,Shmulevich2002}, hierarchical clustering~\cite{JainDubes},
and model-based clustering~\cite{Silvescu01temporalboolean,Smolen2000}. In the general data mining literature, there is a great
proliferation of research on clustering algorithms, in particular
for gene expression data~\cite{Nature_Clustering}. Some of those
studies concentrate both on the ability of an algorithm to obtain a
high quality partition of the data and on its performance in terms
of computational resources, mainly CPU time. For instance,
hierarchical clustering  and K-means algorithms
have been the object of several speedups (see~\cite{Clusterin_high,Kmeanscoresets,Optimal_Hier} and references
therein). Moreover, the need for computational performance is so acute in the area of clustering for microarray data that implementations of well known algorithms, such as K-means, specific for multi-core architectures are being proposed~\cite{Kraus10}.


However, the most fundamental issue to be addressed when clustering data
consists of the determination of the number of clusters. Related
issues are  how to assign confidence levels to the selected number
of clusters, as well as to the induced cluster assignments~\cite{CLEST,Dudoit2003}. Those
issues  are  particularly important and difficult in microarray data
analysis, where the problem of a relatively small sample size is
compounded by the very high dimensionality of the data available,
making the clustering results especially sensitive to noise and
susceptible to over-fitting. Although cluster determination and
assessment are well-known in the classification and statistics
literature and the corresponding methodologies rest on solid
mathematical ground, they are rarely applied to microarray data
analysis tasks. Of relevance here are the so called validation
indices, external, internal and relative, that should assess the
biological relevance of the clustering solutions found.
Internal validation measure evaluate the clusters based solely on the data,
without external information. Typically, a heuristic measure is defined to indicate
the \vir{goodness} of the clustering. 
External validation methods evaluate a clustering algorithm by comparing
the resulting clusters with some \emph{a priori} information~\cite{JainDubes,Tavazoie99}. Agreement between the
heuristic and algorithm-based partitions indicates algorithm accuracy. It also indicates
that the scientific understanding behind the heuristic partition is being reflected
in the measurements, thereby providing supporting evidence for the measurement
process.




Despite the vast amount of knowledge available in this area in the
general data mining literature, e.g.,~\cite{Breckenridge89,
Dudoit2003,Gordon, Gordon1,Tibshrbook,JainDubes,KR90,Kerr00bootstrappingcluster}, gene
expression data provide unique challenges, in particular with
respect to internal validation indices. Indeed, they  must predict
how many clusters are really present in a dataset, an already
difficult task, made even worse by the fact that the estimation must
be sensible enough to capture the inherent biological structure of
functionally related genes. Despite their potentially important
role, both the use of classic internal validation  indices  and the
design of new ones, specific for microarray data, do not seem to
have great prominence in bioinformatics, where attention is mostly
given to clustering algorithms. The excellent survey by Handl et al.~\cite{Handl05} is a big step forward in making the study of those
techniques a central part of both research and practice in
bioinformatics, since it provides both a technical presentation as
well as valuable general guidelines about their use for post-genomic
data analysis. Although much remains to be done, it is,
nevertheless, an initial step.

For instance, in the general data mining literature, there are
several studies, e.g.,~\cite{MC85}, aimed at   establishing  the
intrinsic, as well as the relative, merit of an index. To this end,
the two relevant questions are: (i) What is the precision of an index, i.e., its ability to
predict the correct number of clusters in a dataset? That is usually
established by comparing the number of clusters predicted by the
index against the number of clusters in the true solution of several
datasets, the true solution being a partition of the dataset in
classes that can be trusted to be correct, i.e., distinct groups of
functionally related genes. (ii) Among a collection of indices, which is more accurate, less algorithm dependent,
etc.,?. Precision versus the  use of computational resources,
primarily execution time, would be an important discriminating
factor.
However, for the special case of microarray data, the
experimental assessment of the \vir{fitness} of a measure has been
rather ad hoc and studies in that area provide only partial and
implicit comparison among measures. Moreover, contrary to research
in the clustering literature, the performance of validation methods
in terms of computational resources, again mainly CPU time, is
hardly assessed both in absolute and relative terms.


Having well in mind the two questions above, and in particular for
microarray data, this thesis offers a presentation of some indices
that have been recently proposed and tested on microarray data and
that have gained prominence in the Literature. Obviously, there is
no attempt to be exhaustive and some of the choices of which indices
to include here may be judged as being subjective, although the three most widely known families are taken in account. Namely, indices
based on (a) hypothesis testing in statistics; (b) bootstrapping and
stability techniques and (c) jackknife techniques.
In particular, a deep attention in this thesis is given to the stability based technique. Indeed, during this dissertation a general algorithmic paradigm of them is proposed.

These benchmarks consider both the ability of a measure to predict the correct number
of clusters in a dataset and, departing from the current state of
the art in that area,  the computer time it takes for a measure to
complete its task.
One open question that was made explicit by that study is the  design of a data-driven  internal validation measure
that is both precise and fast, and capable of granting scalability with
dataset size. Such a lack of scalability for the most precise
internal validation measures is one of the main computational
bottlenecks in the process of cluster evaluation for microarray data
analysis. Its elimination is far from trivial~\cite{klie10} and even
partial progress on  this problem is perceived as important.

In terms of the closely related discipline of algorithm theory and
engineering, speedups of that order of magnitude are considered
quite significant. For the microarray data analysis discipline,
although one has not able to close the gap between the time
performance of the fastest validation measures benchmarked or to completely eliminate the bottleneck mentioned
above, the extensive set of experiments conducted in this thesis show a non-trivial step
forward for the solution of those two related problems.

Moreover, this study has some relevance also from the methodological point of
view. First, the idea of \vir{approximating} an internal validation
measure to achieve a speedup with encouraging results. Second, due to the fundamental nature of stability internal validation measures and the ubiquity of their key concepts in the biological data mining
literature, the speedup technique presented here seems applicable to a wider set of measures opening the avenue to a novel
way to gain speed in such an important area of microarray data
analysis. Third, it has also conducted experiments with the use of
Non-negative Matrix Factorization as a clustering algorithm, complementing the
work by Brunet et al.~\cite{BrunetNMF} and Giancarlo et al.~\cite{giancarlo08}. That experiments adds to the state of the art concerning {\tt NMF} a new and important fact: in terms of class discovery {\tt NMF} seems to be worse than hierarchical algorithms both in precision and speed. This fact brings to light, quite clearly, an aspect of {\tt NMF} that may, otherwise, be misleading. Its major virtue is not that of being a clustering algorithm but rather, as pointed out by the ground-breaking work by Brunet et al., and very well summarized in the review by Devarajan, of being an effective tool for pattern discovery in biological data.


\section*{Thesis Contributions}
\addcontentsline{toc}{section}{Thesis Contributions} %\pagenumbering{arabic}

The main contributions of this thesis are the evaluation of internal validations measure in order to infer the \vir{exact} number of clusters in microarrays data.
In particular this study have both theoretical and practical aspect. Indeed, in the first part of the dissertation all the measure used are detailed and a general paradigm of a special class of internal validation measure, i.e., stability based is proposed in the Literature.
The experimental studies, taken in account two main aspect of each measure, i.e.: the precision and the time performance. Based on this analysis it will be evident a hierarchy of the measures taken in account, where the faster measures is a far less precise. For this reason a fundamental aspect of this dissertation is the study of speedup of internal validation measure. Proposing an approximation of five measures and two general schemes of approximation.
Moreover, this thesis also provides for first time in the Literature a benchmark of the Non-negative Matrix Factorization as clustering algorithm on microarray data.


\section*{Thesis Outline}
\addcontentsline{toc}{section}{Thesis Outline} %\pagenumbering{arabic}

The thesis is organized as follows.

\paragraph{Chapter 1} provides the background information relevant to this thesis. Indeed, a formal definition of the clustering problem, and the notation used in this thesis is given. Moreover, the two main classes of clustering algorithms proposed in the literature, some methods for the assessment and evaluation of cluster quality, and data generation/perturbation methods are also detailed.

\paragraph{Chapter 2} provides a presentation of some basic validation techniques. In detail, external and internal indices are outlined. In particular, three external indices that assess the agreement between two partitions, and four internal measures useful to estimate the correct number of clusters present in a dataset, based on: compactness, hypothesis testing in statistics and jackknife techniques are detailed.

\paragraph{Chapter 3} provides one of the main  topics of this thesis. In this chapter internal validation measures based on the notion of stability are presented, and it is introduced a general algorithmic paradigm of them.

\paragraph{Chapter 4} provides a formal description of one of the methodologies that has gained prominence in the data analysis literature: Non-negative Matrix Factorization.

\paragraph{Chapter 5} reviews the experimental environment of this thesis. Here, all the experimental setup used in this dissertation are detailed. Moreover, for the first time in Literature a benchmark of the Non-negative Matrix Factorization as clustering algorithm on microarray data is performed.

\paragraph{Chapter 6} provides a benchmarking of some of the internal validation measures. This study tries to  establish the intrinsic, as well as the relative, merit of a measure taking into account   both its predictive power and its computational demand.

\paragraph{Chapter 7} provides several speedups for four internal validation measures. Moreover, two general approximation schemas are formalized. 
